Hypersuccinct Trees -- New universal tree source codes for optimal compressed tree data structures and range minima

We present a new universal source code for distributions of unlabeled binary and ordinal trees that achieves optimal compression to within lower order terms for all tree sources covered by existing universal codes. At the same time, it supports answering many navigational queries on the compressed representation in constant time on the word-RAM; this is not known to be possible for any existing tree compression method. The resulting data structures, "hypersuccinct trees", hence combine the compression achieved by the best known universal codes with the operation support of the best succinct tree data structures. We apply hypersuccinct trees to obtain a universal compressed data structure for range-minimum queries. It has constant query time and the optimal worst-case space usage of $2n+o(n)$ bits, but the space drops to $1.736n + o(n)$ bits on average for random permutations of $n$ elements, and $2\lg\binom nr + o(n)$ for arrays with $r$ increasing runs, respectively. Both results are optimal; the former answers an open problem of Davoodi et al. (2014) and Golin et al. (2016). Compared to prior work on succinct data structures, we do not have to tailor our data structure to specific applications; hypersuccinct trees automatically adapt to the trees at hand. We show that they simultaneously achieve the optimal space usage to within lower order terms for a wide range of distributions over tree shapes, including: binary search trees (BSTs) generated by insertions in random order / Cartesian trees of random arrays, random fringe-balanced BSTs, binary trees with a given number of binary/unary/leaf nodes, random binary tries generated from memoryless sources, full binary trees, unary paths, as well as uniformly chosen weight-balanced BSTs, AVL trees, and left-leaning red-black trees.

==> universal-succinct-rmq.tex <==
%!TeX root = universal-succinct
\part{Range-Minimum Queries}
\label{part:rmq}

We now show how our tree data structures imply an optimal average-space
solution for the RMQ problem, \ie, 
to the following data structuring task: 
Given an array $A[1..n]$ of comparable items, construct a data structure at preprocessing time that can answer subsequent queries without inspecting $A$ again. 
The answer to the query $\RMQ(i,j)$ for $1\le i\le j\le n$ is the index (in $A$) of the
(leftmost) minimum in $A[i..j]$, \ie,
\[
		\idtt{RMQ}(i,j)
	\wwrel=
		\mathop{\arg\min}\limits_{i\le k\le j} A[k].
\]
We show how to obtain a data structure that answers $\RMQ$ in constant time
using the optimal expected space of $1.736 n + o(n)$ 
bits when the array is a random permutation.
A previous version of this part of the paper, 
containing the results presented below and including more details 
on the data structure aspects of our solution, can be found in \cite{MunroWild2019}.

\section{Preliminaries}


Let $A[1..n]$ store the numbers $x_1,\ldots,x_n$,
\ie, $x_j$ is stored at index $j$ for $1\le j\le n$.
We assume $x_1,\ldots,x_n$ are $n$ distinct numbers;
in case of duplicates, we do not per se require a specific tie breaking rule to be employed.
Duplicates naturally arise, \eg, in the LCE problem, 
but our RMQ solution works regardless which minimum-value index is to be returned.


\subsection{Applications}
\label{sec:rmq-applications}

\todoin{
	All these applications actually need access to the values, as well,
	so it is not quite clear why one would not want to consider the encoding model here.
	Can we find an application where knowing the position is all we want?
}


The RMQ problem is an elementary building block in many data structures.
%It has hence attracted attention in its own right, including the question
%of a data structure with optimal \emph{average-case} space usage.
We discuss two exemplary applications here, in which a non-uniform distribution
over the set of RMQ answers is to be expected.


\todoin{
\paragraph{Document retrieval}
	describe
	
	good thing: genuine application for encoding version
}


\paragraph{Range searching}
A direct application of RMQ data structures lies in 3-sided orthogonal 2D range searching.
Given a set of points in the plane, we maintain an array of the points sorted by $x$-coordinates
and build a range-minimum data structure for the array of $y$-coordinates
and a predecessor data structure for the set of $x$-coordinates.
To report all points in $x$-range $[x_1,x_2]$ and $y$-range $(-\infty, y_1]$,
we find the indices $i$ and $j$ of the outermost points enclosed in $x$-range, \ie, 
the ranks of (the successor of ) $x_1$ resp.\ (the predecessor of) $x_2$.
Then, the range-minimum in $[i,j]$ is the first candidate, 
and we compare its $y$-coordinate to $y_1$.
If it is smaller than $y_1$, we report the point and recurse in both subranges;
otherwise, we stop.

A natural testbed is to consider random point sets.
When $x$- and $y$-coordinates are independent of each other,
the ranking of the $y$-coordinates of points sorted by $x$ form a random permutation, 
and we obtain the exact setting studied in this paper.


\paragraph{Longest-common extensions}
A second application of RMQ data structures is the longest-common extension (LCE) problem on strings:
Given a string/text $T$, the goal is to create a data structure that allows to answer LCE queries,
\ie, given indices $i$ and $j$, what is the largest length $\ell$, so that 
$T_{i,i+\ell-1} = T_{j,j+\ell-1}$.
LCE data structures are a building block, \eg, for finding tandem repeats in genomes;
(see Gusfield's book~\cite{Gusfield1997} for many more applications).


A possible solution is to compute
the suffix array $\mathit{SA}[1..n]$, its inverse $\mathit{SA}^{-1}$, and 
the longest common prefix array $\mathit{LCP}[1..n]$ for the text $T$, where 
$\mathit{LCP}[i]$ stores the length of the longest common prefix of the $i$th and $(i-1)$st 
suffixes of $T$ in lexicographic order.
Using an RMQ data structure on $\mathit{LCP}$, $\mathit{lce}(i,j)$ is found as 
$\mathit{LCP}\bigl[\mathit{rmq}_\mathit{LCP}\bigl(\mathit{SA}^{-1}(i)+1,\mathit{SA}^{-1}(j)\bigr) \bigr]$.
%
%(A classical solution based on lowest common ancestors in the suffix trees 
%is discussed in~\cite{Gusfield1997}.)
\notetoself{
	\url{https://www.sciencedirect.com/science/article/pii/S1570866710000377}
	compared LCE solutions in practice and found that doing either a naive lce by comparing the strings
	or a naive rmq by scanning the range outperforms all constant-time schemes ...
}


Since LCE effectively asks for lowest common ancestors of leaves in suffix trees, %(see \wref{sec:rmq-and-lca}),
the tree shapes arising from this application are related to the shape of the suffix tree of $T$.
This shape heavily depends on the considered input strings, but
for strings generated by a Markov source, it is known that 
random suffix trees behave asymptotically similar to random tries constructed
from independent strings of the same source~\cite[Chap.\,8]{JacquetSzpankowski2015}.
Those in turn have logarithmic height~-- as do random BSTs.
This gives some hope that the RMQ instances arising in the LCE
problem are compressible by similar means.
Indeed, we could confirm the effectiveness of our compression methods
on exemplary text inputs, but further study is needed here.



\notetoself{
	Collection of RMQ applications:
	
	lowest common ancestors in trees,
	longest common extension problem on strings,
	compute suffix links in suffix trees,
	part of compact suffix trees, 
	(3-sided) orthogonal range searching,
	speeding up document retrieval queries,
	finding maximal-scoring subsequences,
	compute Lempel-Ziv-77 factorizations given only the suffix array.
	(those are given in \S3.3 of ``Data Structures for Efficient
	String Algorithms'', Johannes Fischer's dissertation)
	
	moreover from \doi{10.1007/s11786-017-0294-4}
	finding dominators in flow graphs
		(nodes that lie on all paths from the root to a given vertex;
	see \url{https://dl.acm.org/citation.cfm?id=982922}, \doi{10.1016/j.ipl.2008.12.006}),
	position-restricted pattern matching (find matches starting in a range using range next value)
	
}



\subsection{Cartesian Trees}
\label{sec:rmq-cartesian-tree-lca}

The Cartesian tree $T$ for $x_1,\ldots,x_n$ (resp.\ for $A[1..n]$) 
is a binary tree defined recursively as follows:
If $n=0$, it is the empty tree (``null''). 
Otherwise it consists of a root whose left child is the Cartesian tree for $x_1,\ldots,x_{j-1}$
and its right child is the Cartesian tree for $x_{j+1},\ldots,x_n$ where
$j$ is the position of the minimum, $j = \mathop{\arg\min}_k A[k]$;
see \wpref{fig:example-bst} for an example.
A classic observation of Gabow et al.~\cite{GabowBentleyTarjan1984} is that 
range-minimum queries on $A$ are isomorphic to lowest-common-ancestor (LCA) queries on $T$
when identifying nodes with their inorder index:
\[
		\RMQ_A(i,j) 
	\wwrel= 
		\TrRank_{\inorder}\Bigl( 
			\TrLCA_T\bigl(
				\TrSelect_{\inorder}(i),
				\TrSelect_{\inorder}(j)
			\bigr)
		\Bigr).
\]
We can thus reduce an RMQ instance (with arbitrary input) to an LCA instance
of the same size (the number of nodes in $T$ equals the length of the array).
A widely-used reduction from LCA on arbitrary (ordinal) trees to RMQ
writes down the depths of nodes in an Euler tour of the tree.
This produces an RMQ instance of length $2n$ for a tree with $n$ nodes.
However, when $T$ is a \emph{binary} tree, we can replace the Euler tour by a simple 
inorder traversal and thus obtain an RMQ instance of the \emph{same} size.




\section{Random RMQ and Random BSTs}
\label{sec:random-rmq-random-bst}

We consider the random permutation model for RMQ: Every (relative) ordering of
the elements in $A[1..n]$ is considered to occur with the same probability.
Without loss of generality, we identify these $n$ elements with their rank,
\ie, $A[1..n]$ contains a random permutation of $[1..n]$.
We refer to this as a random RMQ instance.

Let $T_n\in\mathcal T_n$ be (the random shape of) the Cartesian tree 
associated with a random RMQ instance (recall \wref{sec:rmq-cartesian-tree-lca}).
We will drop the subscript $n$ when it is clear form the context.
We can precisely characterize the distribution of $T_n$:
Let $t\in\mathcal T_n$ be a given (shape of a) binary tree,
and let $i$ be the inorder index of the root of $t$.
The minimum in a random permutation is located at every position $i\in[n]$ with 
probability $\frac 1n$.
Apart from renaming, the subarrays $A[1..i-1]$ and $A[i+1..n]$ contain a random permutation
of $i-1$ resp. $n-i$ elements, and these two permutations are independent of each other
conditional on their sizes.
We thus have
\begin{align}
\label{eq:rmq-prob-Tn=t-rec}
		\Prob{T_n = t}
	&\wwrel=
		\begin{dcases}
			1, & n \le 1; \\
			\tfrac1n \cdot \Prob{T_{i-1} = t_\ell} \cdot \Prob{T_{n-i} = t_r},
				& n \ge 2,
		\end{dcases}
\end{align}
where $t_\ell$ and $t_r$ are the left resp.\ right subtrees of the root of $t$.
Unfolding inductively yields
\begin{align}
\label{eq:rmq-prob-Tn=t}
		\Prob{T_n = t}
	&\wwrel=
		\prod_{v\in t} \frac1{|t[v]|},
\end{align}
%Note that this is quite far from the uniform distribution over $\mathcal T_n$.
%
where the product is understood to range over all nodes $v$ in $t$.
Recall that $|t[v]|$ denotes the subtree size of $v$.
The very same distribution over binary trees also arises for 
binary search trees (BSTs) when they are built by successive insertions 
from a random permutation (``random BSTs''); recall \wtpref{exm:bst}.
Here, the root's inorder rank is not given by the position of the minimum in the input,
but by the rank of the first element.
That means, the Cartesian tree for a permutation is precisely 
the BST generated by successively inserting the \emph{inverse permutation.}
Since the inverse of a random permutation is itself
distributed uniformly at random over all permutations, 
the resulting tree-shape distributions are the same.



%\begin{lemma}
%The following statements are equivalent from the perspective of the RMQ problem.
%\begin{enumerate}[label=(\roman*)]
%\item $A$ contains a random permutation of $[n]$.
%\item $A$ contains $n$ \iid uniformly in $(0,1)$ distributed real numbers.
%\item Then the min-oriented Cartesian tree on $A$ has the shape distribution
%of a random BST, \ie, the distribution over tree shapes obtained when
%every insertion order is equally likely.
%\end{enumerate}
%\end{lemma}



\subsection{Lower Bound}
\label{sec:rmq-lower-bound}

Since the sets of answers to range-minimum queries is in bijection with Cartesian trees,
the entropy $H_n$ of the distribution of the shape of the Cartesian tree 
gives an information-theoretic lower bound 
for the space required by any RMQ data structure in the encoding model.
For random RMQ instances, we find from \weqref{eq:rmq-prob-Tn=t-rec} and the 
decomposition rule of the entropy that
$H_n$ fulfills the recurrence
\begin{align}
		H_0 \wrel= H_1
	&\wwrel=
		0
\\
		H_n
	&\wwrel=
		\lg n + \frac 1n \sum_{i=1}^n (H_{i-1}+H_{n-i})
		,\qquad(n\ge 2).
\label{eq:rmq-entropy-rec}
\end{align}
We decompose the entropy of the choice of the entire tree shape into 
first choosing the root's rank (entropy $\lg n$ since we uniformly choose between $n$ outcomes)
and adding the entropy for choosing the subtrees conditional on the given subtree sizes.
The above recurrence is very related with recurrences for random binary search trees or 
the average cost in quicksort, only with a different ``toll function''.
Kieffer, Yang and Szpankowski~\cite{KiefferYangSzpankowski2009} show%
\footnote{%
	Hwang and Neininger~\cite{HwangNeininger2002} showed earlier that \weqref{eq:rmq-entropy-rec} can be solved 
	exactly for arbitrary toll functions, and $\lg n$ is one such.%
}
that it
solves to 
\begin{align*}
		H_n 
	&\wwrel= 
		\lg(n) + 2(n+1) \sum_{i=2}^{n-1} \frac{\lg i}{(i+2)(i+1)}
\\	&\wwrel\sim
		2n\sum_{i=2}^{\infty} \frac{\lg i}{(i+2)(i+1)}
\\	&\wwrel\approx 1.7363771 n 
\end{align*}
(Note that Kieffer et al.~use $n$ for the number of external leaves, where we count (internal) nodes, 
so there is an off-by-one in the meaning of $n$.)
%
The asymptotic approximation is actually a fairly conservative upper bound for small $n$, see
\wref{fig:rmq-entropy}.

\begin{figure}[hbt]
	\mathematicaPlotPdf{average-bst-entropy-over-n}
	\caption{%
		$H_n/n$ (blue) and its limit $\lim_{n\to\infty} H_n/n \approx 1.736$ (yellow) for $n\le 100$.
	}
\label{fig:rmq-entropy}
\end{figure}


\subsection{Putting it All Together}

With these preparations, we are ready to prove our main result on range-minimum queries.

\begin{theorem}[Average-case optimal succinct RMQ]
\label{thm:avg-space-rmq}
	There is a data structure that supports (static) range-minimum queries on an array $A$ of 
	$n$ (distinct) numbers in $\Oh(1)$ worst-case time and which
	occupies $H_n + o(n) \approx 1.736 n + o(n)$
	bits of space on average over all possible permutations of the elements in $A$.
	The worst-case space usage is $2n + o(n)$ bits.
\end{theorem}

\begin{proof}
The shapes of Cartesian trees build on random permutations are produced by the monotonic 
fixed-size source of \wref{exm:bst}; by \wref{thm:binary-monotonic-fixed-size},
our hypersuccinct code has maximal pointwise redundancy of $o(n)$, hence also
$o(n)$ expected redundancy.
Using the hypersuccinct code in \wref{thm:binary-tree-covering}, we obtain a tree data structure
supporting in particular $\TrRank_{\inorder}$, $\TrSelect_{\inorder}$ and $\TrLCA$,
thus we can answer $\RMQ$ in constant time.
Averaging the instance-specific space $\lg(1/\Prob t)$ over all binary trees $t\in\mathcal T_n$
yields the source entropy, $H_n\sim 1.736 n$.
Since the hypersuccinct code uses length-bounded Huffman codes, we never use more than $2n+o(n)$ bits
on any input.
\end{proof}

We note that our data structure immediately extends to other possible 
shape distributions of Cartesian trees as long as they can we written as on of the sources
listed in \wref{sec:contributions}.
